DLHT: A Non-blocking Resizable Hashtable with Fast Deletes and Memory-awareness

This paper presents DLHT, a concurrent in-memory hashtable. Despite efforts to optimize hashtables, that go as far as sacrificing core functionality, state-of-the-art designs still incur multiple memory accesses per request and block request processing in three cases. First, most hashtables block while waiting for data to be retrieved from memory. Second, open-addressing designs, which represent the current state-of-the-art, either cannot free index slots on deletes or must block all requests to do so. Third, index resizes block every request until all objects are copied to the new index. Defying folklore wisdom, DLHT forgoes open-addressing and adopts a fully-featured and memory-aware closed-addressing design based on bounded cache-line-chaining. This design offers lock-free index operations and deletes that free slots instantly, (2) completes most requests with a single memory access, (3) utilizes software prefetching to hide memory latencies, and (4) employs a novel non-blocking and parallel resizing. In a commodity server and a memory-resident workload, DLHT surpasses 1.6B requests per second and provides 3.5x (12x) the throughput of the state-of-the-art closed-addressing (open-addressing) resizable hashtable on Gets (Deletes).

==> 0_sections/7_discussion.tex <==
\section{Discussion}
\begin{comment}
\beginbsec{Context}
\begin{itemize}
    \item in-memory storage: cache-optimized but memory-resident working set
    \item loss-less index: not just a cache (e.g., like MICA)
\end{itemize}

\beginbsec{Features}
\begin{itemize}
\item >1 billion ops on commodity x86 and Arm (Huawei's Kungpeng) servers, following sequential proximity. 
\item extreme throughput, scalable, h/w - s/w co-design
\end{itemize}


\beginbsec{Programmable}
\begin{itemize}
\item Agile Interface: Hashset, Ptr API, batching (same and across hts), external prefetching, tx API (i.e., shadow inserts), hashtable ids
\item Strongest Consistency: Linearizable CRUD, 
\item Use cases: lock manager, KV storage, transactional storage, knobs
\end{itemize}


\beginbsec{Why Mimalloc?}
\begin{itemize}
\item multi-size allocations
\item high-performance (100M AP), huge pages, socket pinning, etc.
\item producer/consumer (asymmetric) alloc/free
\end{itemize}

\beginbsec{Future-proof}
\begin{itemize}
\item Protocol agnostic: decoupled cc/tx protocols
\item Designed while keeping in mind: persistence, MVCC, CXL(?), h/w acceleration, distributed setup etc.
\end{itemize}


\beginbsec{Performant (high-throughput (100s MIOPs, latency below an SLO))}
\begin{itemize}
\item Highly concurrent: scale to multiple threads (>40), across numa nodes, symmetric design
\item Synchronization 1: wait-free/lock-free index operations: up to 4 chained buckets (unlike 1 bucket of CLHT)
\item Synchronization 2: non-blocking resizing (operations complete with strong consistency during resizing)
\item Cache-awareness: false-sharing, cache alignment, minimized coherence traffic (e.g., write-free operation with no coherence cost)
\item Memory accesses: reduced accesses and masked latency (via batching + s/w prefetching)
\end{itemize}



\beginbsec{Low-level Features:}
\begin{itemize}
\item variable-sized keys and (unique inlined) values or pointers (to values with requested alignment), 4B pointers, Garbage Collection
\item DLHT is broken down to HtIndex and DStore: the app never acquires locks in HtIndex.
\item iterator (strongly consistent and not)
\end{itemize}


\beginbsec{Hashing}
\begin{itemize}
\item disabled/enabled, internal, external (caching hashes to avoid recomputing them)
\item never hash keys more than once
\item evaluate several different hashes. Is hybrid the best one?
\end{itemize}

\beginbsec{Allocations}
\begin{itemize}
\item index: Adaptive small-page to huge-pages pinned index
\item objects: A highly-performing (100M alloc/frees per sec of 64B) memory allocator. Desired features: Multi-size allocation support, huge pages, asymmetric alloc/free (one thread may free an object allocated by another thread) --> Mimalloc, mm (for 4B compressed ptrs) 
\item Epoch-based GC (necessary for lock-free data structures, MVCC, pointer-exposed API etc.)
Multi-size allocation support
\item in-lined unique values. 
\end{itemize}

\beginbsec{Could also explore}
\begin{itemize}
\item experiment over RDMA
\item power over arm
\item CXL, persistency
\item design for compressed index e.g., 4B keys and ptrs
\item key resizing hints (to avoid recomputing hashes)
\item ht contract (resizing) 
\item aHash (use its smhash folder library)
\item small scans (no hashing, <= 8B keys)
\item iterator (?)
\item strongest consistency snapshots (utilize resizing)
\item what is the largest ht size (i.e., number of stored keys) with decent performance?
\item inserting a given ptr or a given inlined value <= X bytes (instead of allocating new memory).
\end{itemize}


\subsection{Related work}

\beginbsec{CLHT [ASPLOS'15]}
\begin{itemize}
\item [+] Lossless index
\item [+] Cache-awareness (write-free operations --> no coherence cost)
\item [+] Wait-free/Lock-free index operations
\item [-] Limited API: Put = Del -> Ins (costly and not linearizable Del + Insert are not atomic)
\item [-] Cache-resident focus (target workload: 4k Objects)
\end{itemize}



\beginbsec{MICA++ [ISCA'15, TOCS'16]}
\begin{itemize}
\item [-] Primarily Lossy index (e.g., to be used as an in-memory cache)
\item [+] CRUD API
\item [+] Memory resident
\item [+] Batching + s/w prefetching
\item [-] CC: Lock-based / EREW (prone to skew --> not thread scalable)
\end{itemize}


\beginbsec{TODO}
\begin{itemize}
\item MICA, CLHT, 
\item shrink
\item memory usage
\end{itemize}
\end{comment}

==> 3_incl_graphics/eval_join.tex <==
\begin{figure}[t]
\vspace{-3pt}
% \hspace{-3pt}
% \includegraphics[width=0.33\textwidth]{2_graphs/Join.pdf}
\includegraphics[width=0.33\textwidth]{2_graphs/JoinThreads.pdf}
\vspace{-10pt}
% \caption{Throughput of non-partitioned Hash Join over DLHT with build relation of ${}$tuples while varying probe relation size.}
\caption{Throughput while varying threads of Hash Join -- build relation of $2^{27}$ tuples | probe relation of $2^{31}$ tuples.}
\vspace{-15pt}
\label{fig:join}

\end{figure}

==> 3_incl_graphics/table_baselines.tex <==
% \begin{table}[t]
\resizebox{1.1\linewidth}{!}{% use resizebox with textwidth
% \hspace{-35pt}
% \begin{tabularx}{2.\linewidth}{X}
% \centering
% \begin{tabular}{|l|l}
\begin{tabular}{l|l}
% \hline
\textbf{CLHT} & lock-free variant of CLHT~\cite{Tudor:15, Tudor:14} \\
\textbf{MICA} & CRCW variant of MICA2~\cite{Li:2015, Li:2016} \\
\textbf{GrowT} & uaGrowT variant of GrowT~\cite{Maier:19} \\
\textbf{Folly} & Meta's Folly atomic map~\cite{Folly:23} \\
\textbf{Cuckoo} & concurrent Cuckoo hash map~\cite{Fan:2013} \\
\textbf{Leapfrog} & Leapfrog map of Junction lib~\cite{Leapfrog:16} \\
\textbf{TBB} & Intel's OneTBB concurrent map~\cite{TBB:23} \\
\textbf{DRAMHiT} & lock-free open-addressing map~\cite{Narayanan:23} \\
\textbf{\dlht(-NoBatch)} & as in \cref{sec:design} (without batching -- \cref{sec:des:batch})
\\ 
% \hline
\end{tabular}
% \end{tabularx}
}

% \vspace{-5pt}
\vspace{5pt}
\captionof{table}{Evaluated Hashtables}
% \caption{Evaluated Hashtables.}
\label{tab:base}
% \vspace{-25pt}
% \end{table}

==> 3_incl_graphics/table_core_features.tex <==
\begin{table}[]
\resizebox{1\linewidth}{!}{% use resizebox with textwidth
\begin{tabularx}{2.2\linewidth}{X}
\begin{tabular}{l|l|lllll|ll|l|}
\cline{2-10}
 &
   &
  \multicolumn{5}{l|}{\textbf{Parallel and Non-blocking (core functionality)}} &
  \multicolumn{2}{l|}{\textbf{Memory accesses}} &
  \textbf{Extra features} \\ \cline{3-10} 
\multirow{-2}{*}{} &
  \multirow{-2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Probing  \\ (collision \\ handling)\end{tabular}}} &
  \multicolumn{1}{l|}{\textbf{Gets}} &
  \multicolumn{1}{l|}{\textbf{Puts}} &
  \multicolumn{1}{l|}{\textbf{Inserts}} &
  \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Deletes\\ (that free \\ index slots)\end{tabular}}} &
  \textbf{Resizes} &
  \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Software \\ prefetch\end{tabular}}} &
  \textbf{\begin{tabular}[c]{@{}l@{}}Index \\inlining\\ support\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}l@{}}kv pairs \textgreater 16B, \\ namespaces,\\ 1-thread and \\ tnx. aware\end{tabular}} \\ \hline
\multicolumn{1}{|l|}{\textbf{\begin{tabular}[c]{@{}l@{}}DLHT \\ \end{tabular}}} &
  \begin{tabular}[c]{@{}l@{}}closed addressing \\ (cacheline chains \\  + resize)\end{tabular} &
  \multicolumn{1}{l|}{{\color[HTML]{036400} V}} &
  \multicolumn{1}{l|}{{\color[HTML]{036400} V}} &
  \multicolumn{1}{l|}{{\color[HTML]{036400} V}} &
  \multicolumn{1}{l|}{{\color[HTML]{036400} V}} &
  {\color[HTML]{036400} \begin{tabular}[c]{@{}l@{}}V (Parallel, \\ non-blocking -- \\ safe ops \\ during resize)\end{tabular}} &
  \multicolumn{1}{l|}{{\color[HTML]{036400} V}} &
  {\color[HTML]{036400} V} &
  {\color[HTML]{036400} V} \\ \hline
\multicolumn{1}{|l|}{\textbf{\begin{tabular}[c]{@{}l@{}}CLHT\end{tabular}}} &
  \begin{tabular}[c]{@{}l@{}}closed addressing\\ (1-cacheline \\ + resize)\end{tabular} &
  \multicolumn{1}{l|}{{\color[HTML]{036400} V}} &
  \multicolumn{1}{l|}{{\color[HTML]{9A0000} X}} &
  \multicolumn{1}{l|}{{\color[HTML]{036400} V}} &
  \multicolumn{1}{l|}{{\color[HTML]{036400} V}} &
  {\color[HTML]{9A0000} \begin{tabular}[c]{@{}l@{}}Serial, \\ Blocking\end{tabular}} &
  \multicolumn{1}{l|}{{\color[HTML]{CE6301} X}} &
  {\color[HTML]{036400} V} &
  {\color[HTML]{9A0000} X} \\ \hline
  \multicolumn{1}{|l|}{\textbf{MICA}} &
  \begin{tabular}[c]{@{}l@{}}closed addressing \\ (cacheline chains)\end{tabular} &
  \multicolumn{1}{l|}{{\color[HTML]{036400} V}} &
  \multicolumn{1}{l|}{{\color[HTML]{CE6301} \begin{tabular}[c]{@{}l@{}}Block\\ -ing\end{tabular}}} &
  \multicolumn{1}{l|}{{\color[HTML]{CE6301} Blocking}} &
  \multicolumn{1}{l|}{{\color[HTML]{CE6301} Blocking}} &
  {\color[HTML]{9A0000} X} &
  \multicolumn{1}{l|}{{\color[HTML]{036400} V}} &
  {\color[HTML]{680100} \begin{tabular}[c]{@{}l@{}}X (\textgreater{}=2 \\memory\\      accesses)\end{tabular}} &
  {\color[HTML]{CD9934} kv pairs \textgreater 16B} \\ \hline
\multicolumn{1}{|l|}{\textbf{GrowT}} &
  \begin{tabular}[c]{@{}l@{}}open addressing\\ (linear probing \\ + resize)\end{tabular} &
  \multicolumn{1}{l|}{{\color[HTML]{036400} V}} &
  \multicolumn{1}{l|}{{\color[HTML]{036400} V}} &
  \multicolumn{1}{l|}{{\color[HTML]{036400} V}} &
  \multicolumn{1}{l|}{{\color[HTML]{9A0000} \begin{tabular}[c]{@{}l@{}}Blocking \\(until all index \\is transferred)\end{tabular}}} &
  {\color[HTML]{CE6301} \begin{tabular}[c]{@{}l@{}}Parallel,\\ Blocking\end{tabular}} &
  \multicolumn{1}{l|}{{\color[HTML]{CE6301} X}} &
  {\color[HTML]{036400} V} &
  {\color[HTML]{9A0000} X} \\ \hline
\multicolumn{1}{|l|}{\textbf{Folly}} &
  \begin{tabular}[c]{@{}l@{}}open addressing \\ (linear probing)\end{tabular} &
  \multicolumn{1}{l|}{{\color[HTML]{036400} V}} &
  \multicolumn{1}{l|}{{\color[HTML]{036400} V}} &
  \multicolumn{1}{l|}{{\color[HTML]{036400} V}} &
  \multicolumn{1}{l|}{{\color[HTML]{9A0000} Cannot free}} &
  {\color[HTML]{9A0000} X} &
  \multicolumn{1}{l|}{{\color[HTML]{CE6301} X}} &
  {\color[HTML]{036400} V} &
  {\color[HTML]{9A0000} X} \\ \hline
% \multicolumn{1}{|l|}{\textbf{Intel TBB}} &
%   chained hashing &
%   \multicolumn{1}{l|}{X} &
%   \multicolumn{1}{l|}{} &
%   \multicolumn{1}{l|}{} &
%   \multicolumn{1}{l|}{X} &
%   X &
%   \multicolumn{1}{l|}{X} &
%    &
%   V \\ \hline
% \multicolumn{1}{|l|}{\textbf{Cuckoo}} &
%   cuckoo hashing &
%   \multicolumn{1}{l|}{X} &
%   \multicolumn{1}{l|}{} &
%   \multicolumn{1}{l|}{} &
%   \multicolumn{1}{l|}{blocking} &
%   X &
%   \multicolumn{1}{l|}{X} &
%    &
%   V \\ \cline{1-8} \cline{10-10} 
% \multicolumn{1}{|l|}{\textbf{Leapfrog}} &
%   hopscotch hashing &
%   \multicolumn{1}{l|}{V} &
%   \multicolumn{1}{l|}{} &
%   \multicolumn{1}{l|}{} &
%   \multicolumn{1}{l|}{blocking} &
%    &
%   \multicolumn{1}{l|}{X} &
%    &
%   V \\ \cline{1-8} \cline{10-10} 
\end{tabular}
\end{tabularx}
}
\end{table}

==> 3_incl_graphics/table_core_features2.tex <==
\begin{table}[]
\resizebox{1\linewidth}{!}{% use resizebox with textwidth
\begin{tabularx}{1.9\linewidth}{X}
\begin{tabular}{l|l|lllll|ll|}
\cline{2-9}
 &
   &
  \multicolumn{5}{l|}{\textbf{Non-blocking}} &
  \multicolumn{2}{l|}{\textbf{Memory accesses}} \\ \cline{3-9} 
\multirow{-2}{*}{} &
  \multirow{-2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Probing  \\ (collision\\  handling)\end{tabular}}} &
  \multicolumn{1}{l|}{\textbf{Gets}} &
  \multicolumn{1}{l|}{\textbf{Puts}} &
  \multicolumn{1}{l|}{\textbf{Inserts}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\textbf{Deletes}\\ (that free \\ index slots)\end{tabular}} &
  \begin{tabular}[c]{@{}l@{}}\textbf{Resizes}\\ (Non-blocking \\ = safe op exec. \\ during resize)\end{tabular} &
  \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Software\\ prefetch\end{tabular}}} &
  \textbf{\begin{tabular}[c]{@{}l@{}}Index \\ inlining \\ support\end{tabular}} \\ \hline
\multicolumn{1}{|l|}{\textbf{DLHT}} &
  \begin{tabular}[c]{@{}l@{}}close addressing \\ (cacheline chains \\  + resize)\end{tabular} &
  \multicolumn{1}{l|}{{\color[HTML]{036400} \cmark}} &
  \multicolumn{1}{l|}{{\color[HTML]{036400} \cmark}} &
  \multicolumn{1}{l|}{{\color[HTML]{036400} \cmark}} &
  \multicolumn{1}{l|}{{\color[HTML]{036400} \cmark}} &
  {\color[HTML]{036400} \cmark} &
  \multicolumn{1}{l|}{{\color[HTML]{036400} \cmark}} &
  {\color[HTML]{036400} \cmark} \\ \hline
\multicolumn{1}{|l|}{\textbf{CLHT}} &
  \begin{tabular}[c]{@{}l@{}}close addressing\\ (single-cacheline\\  + resize)\end{tabular} &
  \multicolumn{1}{l|}{{\color[HTML]{036400} \cmark}} &
  \multicolumn{1}{l|}{{\color[HTML]{9A0000} \xmark}} &
  \multicolumn{1}{l|}{{\color[HTML]{036400} \cmark}} &
  \multicolumn{1}{l|}{{\color[HTML]{036400} \cmark}} &
  {\color[HTML]{9A0000} \begin{tabular}[c]{@{}l@{}}Serial, \\ Blocking\end{tabular}} &
  \multicolumn{1}{l|}{{\color[HTML]{9A0000} \xmark}} &
  {\color[HTML]{036400} \cmark} \\ \hline
\multicolumn{1}{|l|}{\textbf{MICA}} &
  \begin{tabular}[c]{@{}l@{}}close addressing \\ (cacheline chains)\end{tabular} &
  \multicolumn{1}{l|}{{\color[HTML]{036400} \cmark}} &
  \multicolumn{1}{l|}{{\color[HTML]{F56B00} \begin{tabular}[c]{@{}l@{}}Block-\\ ing\end{tabular}}} &
  \multicolumn{1}{l|}{{\color[HTML]{F56B00} \begin{tabular}[c]{@{}l@{}}Block-\\ ing\end{tabular}}} &
  \multicolumn{1}{l|}{{\color[HTML]{F56B00} Blocking}} &
  {\color[HTML]{9A0000} \xmark} &
  \multicolumn{1}{l|}{{\color[HTML]{036400} \cmark}} &
  % {\color[HTML]{9A0000} \begin{tabular}[c]{@{}l@{}}\xmark (\textgreater{}=2 mem.\\      accesses)\end{tabular}} \\ \hline
  {\color[HTML]{9A0000} \begin{tabular}[c]{@{}l@{}}\xmark\end{tabular}} \\ \hline
\multicolumn{1}{|l|}{\textbf{GrowT}} &
  \begin{tabular}[c]{@{}l@{}}open addressing\\ (linear probing \\ + resize)\end{tabular} &
  \multicolumn{1}{l|}{{\color[HTML]{036400} \cmark}} &
  \multicolumn{1}{l|}{{\color[HTML]{036400} \cmark}} &
  \multicolumn{1}{l|}{{\color[HTML]{036400} \cmark}} &
  \multicolumn{1}{l|}{{\color[HTML]{9A0000} \begin{tabular}[c]{@{}l@{}}Blocking \\ (until all index \\ is transferred)\end{tabular}}} &
  {\color[HTML]{F56B00} \begin{tabular}[c]{@{}l@{}}Parallel,\\ Blocking\end{tabular}} &
  \multicolumn{1}{l|}{{\color[HTML]{9A0000} \xmark}} &
  {\color[HTML]{036400} \cmark} \\ \hline
\multicolumn{1}{|l|}{\textbf{Folly}} &
  \begin{tabular}[c]{@{}l@{}}open addressing \\ (quadratic prob.)\end{tabular} &
  \multicolumn{1}{l|}{{\color[HTML]{036400} \cmark}} &
  \multicolumn{1}{l|}{{\color[HTML]{036400} \cmark}} &
  \multicolumn{1}{l|}{{\color[HTML]{036400} \cmark}} &
  \multicolumn{1}{l|}{{\color[HTML]{9A0000} Cannot free}} &
  {\color[HTML]{9A0000} \xmark} &
  \multicolumn{1}{l|}{{\color[HTML]{9A0000} \xmark}} &
  {\color[HTML]{036400} \cmark} \\ \hline
\end{tabular}
\end{tabularx}
}
\caption{Comparison of features between DLHT and fastest state-of-the-art baselines.}
\label{tab:features}
\end{table}

==> 3_incl_graphics/table_feature_backup.tex <==
\begin{table*}[t]
% \hspace{-25pt}
\resizebox{0.79\linewidth}{!}{% use resizebox with textwidth
% \begin{tabularx}{1.65\linewidth}{X}
% \resizebox{2\linewidth}{!}{% use resizebox with textwidth
% \begin{tabularx}{2\linewidth}{XX}
\begin{tabular}{l|lllll|lll|}
% \cline{2-8}
 % &
 % probing
 &
  \multicolumn{5}{c|}{\textbf{Practically non-blocking operations}} &
  \multicolumn{3}{c}{\textbf{Memory access awareness}} \\ \cline{2-9} 
\multirow{-2}{*}{} &
  \multicolumn{1}{c}{\textbf{Gets}} &
  \multicolumn{1}{c}{\textbf{Puts}} &
  \multicolumn{1}{c}{\textbf{Inserts}} &
  \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}} \textbf{Deletes}\\ (that free \\ index slots)\end{tabular}} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Resizes}\\ (non-blocking:\\ safe Get,..,Del \\ during resize)\end{tabular}} &
  \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}} \textbf{Overlaps}\\ \textbf{memory accesses}\\ (i.e., exploits \\ s/w prefetch)\end{tabular}} &
  \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}} \textbf{Minimizes} \\ \textbf{memory traffic} \\ (e.g., supports\\ index inlining)\end{tabular}} &
  \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}} \textbf{Occupancy} \\ until resize \\ (from \cref{sec:eval:occupancy}\\ with wyhash)\end{tabular}} \\ 
  % \hline
  % \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Index \\ inlining \\ support\end{tabular}}} \\ \hline
  \hlinewd{3pt}
\multicolumn{1}{l|}{\textbf{MICA}} &
% \multicolumn{1}{l|}{\textbf{MICA}} &
  \multicolumn{1}{c}{{\color[HTML]{036400} \cmark}} &
  \multicolumn{1}{c}{{\color[HTML]{F56B00} \begin{tabular}[c]{@{}c@{}}Blocking\end{tabular}}} &
  \multicolumn{1}{c}{{\color[HTML]{F56B00} \begin{tabular}[c]{@{}c@{}}Blocking\end{tabular}}} &
  \multicolumn{1}{c}{{\color[HTML]{F56B00} Blocking}} &
  \multicolumn{1}{c|}{{\color[HTML]{9A0000} \xmark}} &
  \multicolumn{1}{c}{{\color[HTML]{036400} \cmark}} &
  % {\color[HTML]{90000} \begin{tabular}[c]{@{}l@{}}\xmark (\textgreater{}=2 mem.\\      accesses)\end{tabular}} \\ \hline
  \multicolumn{1}{c}{{\color[HTML]{9A0000} \xmark}} &
  \multicolumn{1}{c}{{\color[HTML]{9A0000} \textbf{---}}} \\ \hline
\multicolumn{1}{l|}{\textbf{CLHT}} &
% \multicolumn{1}{l|}{\textbf{CLHT}} &
  \multicolumn{1}{c}{{\color[HTML]{036400} \begin{tabular}[c]{@{}c@{}}{\color[HTML]{F56B00}Unique values}\end{tabular}}} &
  \multicolumn{1}{c}{{\color[HTML]{9A0000} \xmark}} &
  \multicolumn{1}{c}{{\color[HTML]{036400} \cmark}} &
  \multicolumn{1}{c}{{\color[HTML]{036400} \cmark}} &
  \multicolumn{1}{c|}{{\color[HTML]{9A0000} \begin{tabular}[c]{@{}c@{}}Serial, \\ Blocking\end{tabular}}} &
  \multicolumn{1}{c}{{\color[HTML]{9A0000} \xmark}} &
  \multicolumn{1}{c}{{\color[HTML]{036400} \cmark}} &
  \multicolumn{1}{c}{{\color[HTML]{9A0000} \textbf{5\%}}} \\ \hline
  % \multicolumn{1}{c}{{\color[HTML]{036400} \cmark}} \\ \hline
\multicolumn{1}{l|}{\textbf{GrowT}} &
% \multicolumn{1}{l|}{\textbf{GrowT}} &
  \multicolumn{1}{c}{{\color[HTML]{036400} \cmark}} &
  \multicolumn{1}{c}{{\color[HTML]{036400} \cmark}} &
  \multicolumn{1}{c}{{\color[HTML]{036400} \cmark}} &
  \multicolumn{1}{c}{{\color[HTML]{9A0000} \begin{tabular}[c]{@{}c@{}}Blocking \\ (until all index \\ is transferred)\end{tabular}}} &
  \multicolumn{1}{c|}{{\color[HTML]{F56B00} \begin{tabular}[c]{@{}c@{}}Parallel,\\ Blocking\end{tabular}}} &
  \multicolumn{1}{c}{{\color[HTML]{9A0000} \xmark}} &
  \multicolumn{1}{c}{{\color[HTML]{036400} \cmark}} &
  \multicolumn{1}{c}{{\color[HTML]{F56B00} \textbf{30\%}}} \\ \hline
\multicolumn{1}{l|}{\textbf{Folly}} &
% \multicolumn{1}{l|}{\textbf{Folly}} &
  \multicolumn{1}{c}{{\color[HTML]{036400} \cmark}} &
  \multicolumn{1}{c}{{\color[HTML]{036400} \cmark}} &
  \multicolumn{1}{c}{{\color[HTML]{036400} \cmark}} &
  \multicolumn{1}{c}{{\color[HTML]{9A0000} \xmark}} &
  \multicolumn{1}{c|}{{\color[HTML]{9A0000} \xmark}} &
  \multicolumn{1}{c}{{\color[HTML]{9A0000} \xmark}} &
  \multicolumn{1}{c}{{\color[HTML]{036400} \cmark}} &
  \multicolumn{1}{c}{{\color[HTML]{9A0000} \textbf{---}}} \\ \hline
\multicolumn{1}{l|}{\textbf{\begin{tabular}[l]{@{}l@{}}DRAMHiT\\\scalebox{0.78}{(concur. work)}\end{tabular}}
% \multicolumn{1}{l|}{\textbf{\begin{tabular}[l]{@{}l@{}}DRAMHiT\\\scalebox{0.78}{(concur. work)}\end{tabular}}
} &
  \multicolumn{1}{c}{{\color[HTML]{036400} \cmark}} &
  \multicolumn{1}{c}{{\color[HTML]{036400} \begin{tabular}[c]{@{}c@{}}{\color[HTML]{F56B00}Only upsert}\end{tabular}}} &
  \multicolumn{1}{c}{{\color[HTML]{036400} \begin{tabular}[c]{@{}c@{}}{\color[HTML]{F56B00}Only upsert}\end{tabular}}} &
  % \multicolumn{1}{c}{{\color[HTML]{036400} \begin{tabular}[c]{@{}c@{}}\cmark\\ {\color[HTML]{F56B00}(only upsert)}\end{tabular}}} &
  \multicolumn{1}{c}{{\color[HTML]{9A0000} \xmark}} &
  \multicolumn{1}{c|}{{\color[HTML]{9A0000} \xmark}} & 
  \multicolumn{1}{c}{{\color[HTML]{F56B00} \begin{tabular}[c]{@{}c@{}} Reorders requests\end{tabular}}} &
  \multicolumn{1}{c}{{\color[HTML]{036400} \cmark}} &
  \multicolumn{1}{c}{{\color[HTML]{9A0000} \textbf{---}}} \\ \hlinewd{3pt}
  \multicolumn{1}{l|}{\textbf{DLHT}} &
  % \multicolumn{1}{l|}{\textbf{DLHT}} &
  \multicolumn{1}{c}{{\color[HTML]{036400} \cmark}} &
  \multicolumn{1}{c}{{\color[HTML]{036400} \cmark}} &
  \multicolumn{1}{c}{{\color[HTML]{036400} \cmark}} &
  \multicolumn{1}{c}{{\color[HTML]{036400} \cmark}} &
  \multicolumn{1}{c|}{{\color[HTML]{036400} \cmark}} &
  \multicolumn{1}{c}{{\color[HTML]{036400} \cmark}} &
  \multicolumn{1}{c}{{\color[HTML]{036400} \cmark}} &
  \multicolumn{1}{c}{{\color[HTML]{036400} \textbf{70\%}}} \\ 
  % \hline
\end{tabular}
% \end{tabularx}
} % resizebox end
\vspace{5pt}
% \caption{State-of-the-art concurrent hashtables and \dlht\ support of key performance features for memory-resident usage.}
\caption{Key features for memory-resident performance across state-of-the-art concurrent in-memory hashtables and \dlht.}
\label{tab:core_features}
\vspace{-20pt}
\end{table*}

==> 3_incl_graphics/table_features_old.tex <==
\begin{table*}[ht]
\resizebox{1.7\linewidth}{!}{% use resizebox with textwidth
\begin{tabularx}{2\linewidth}{X}
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
 &
  Type &
  \begin{tabular}[c]{@{}l@{}}Supports: deletes*, \\ index resizing, \\ and variable-size \\ key-value pairs\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}lock-free\\ index\\ operations\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Non-blocking \\ resizing\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Masks \\ memory\\ accesses\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Agile \\ Thrifty\\ Interface\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Performance\\ not subject to (e.g.,\\ dwCAS, HTM, \\ SIMD, flow-steer)\end{tabular} \\ \hline
DLHT (this work)             & cache-line chaining & V & V               & V & V & V      & V                             \\ \hline
MICA++                       & fixed size          & X & X               & X & V & X      & flow-steer (-EREW) \\ \hline
CLHT                         & cache-line chaining & X & V (-lf variant) & X & X & X      & V                             \\ \hline
uaGrowT                      & linear probing      & X & needs dwCAS     & V & X & $\sim$ & X (dwCAS/HTM)                 \\ \hline
FolkloreHt                   & linear probing      & X & needs dwCAS     & X & X & X      & X (dwCAS/HTM)                 \\ \hline
Facebook Folly               & linear probing      & X & X               & X & X & X      & X (SIMD)                      \\ \hline
Intel TBB                    & chained hashing     & V & X               & X & X & X      & V                             \\ \hline
Cuckoo                       & cuckoo hashing      & V & X               & X & X & X      & V                             \\ \hline
Leapfrog                     & hopscotch hashing variant   & V & V               & ? & X & X      & V                             \\ \hline
\end{tabular}
\end{tabularx}
}
\caption{TBD.}
\label{tab:features}
\end{table*}

==> 3_incl_graphics/table_ycsb.tex <==
\begin{table}[t!]

\resizebox{0.69\columnwidth}{!}{% use resizebox with textwidth
\begin{tabular}{l|lrrr}
 &
  \textbf{Characteristic} &
  \multicolumn{1}{l}{\textbf{Gets}} &
  \multicolumn{1}{l}{\textbf{Puts}} &
  \multicolumn{1}{l}{\textbf{RMWs}} \\ \cline{2-5} 
\textbf{YCSB A} & PutHeavy & 50\% & 50\% & \\
\textbf{YCSB B} & GetHeavy & 95\%  & 5\% & \\
\textbf{YCSB C} & Get(-only)  &  100\% & & \\
\textbf{YCSB F} & RMWs(-only) &  & & 100\% \\
\end{tabular}
}

\caption{Summary of evaluated (single-key) YCSB mixes.}
\vspace{-25pt}
\label{tab:ycsb}
\end{table}

==> Makefile <==
#
## Makefile for acmart package
#

PACKAGE=acmart

MAIN_TEX=paper


TEXSRCS := $(wildcard *.tex) \
	   $(wildcard ./0_sections/*.tex) \
	   $(wildcard ./3_misc/*.tex) \
	   $(wildcard ./4_incl_graphics/*.tex)


all:  $(MAIN_TEX).pdf

%.cls:   %.ins %.dtx  
		pdflatex $<

$(MAIN_TEX).pdf:  $(PACKAGE).cls ACM-Reference-Format.bst $(TEXSRCS)
		pdflatex $(MAIN_TEX)
		- bibtex $(MAIN_TEX)
		pdflatex $(MAIN_TEX)
		pdflatex $(MAIN_TEX)

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

clean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi

pdf-clean: clean
	$(RM) $(MAIN_TEX).pdf

